Analysis of a Stochastic Switched Model of Freeway Traffic Incidents

This article introduces a model for freeway traffic dynamics under stochastic capacity-reducing incidents, and provides insights for freeway incident management by analyzing long-time (stability) properties of the proposed model. Incidents on a multi-cell freeway are modeled by reduction in capacity at the affected freeway sections, which occur and clear according to a Markov chain. We develop conditions under which the traffic queue induced by stochastic incidents is bounded. A necessary condition is that the demand must not exceed the time-average capacity adjusted for spillback. A sufficient condition, in the form of a set of bilinear inequalities, is also established by constructing a Lyapunov function and applying the classical Foster-Lyapunov drift condition. Both conditions can be easily verified for realistic instances of the stochastic incident model. Our analysis relies on the construction of a globally attracting invariant set, and exploits the properties of the traffic flow dynamics. We use our results to analyze the impact of stochastic capacity fluctuation (frequency, intensity, and spatial correlation) on the throughput of a freeway segment.

==> Sections/80_Biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Jin.jpg}}]{Li Jin}
is a Ph.D. candidate in Transportation at the Massachusetts Institute of Technology (MIT).  He received the B.Eng. degree from Shanghai Jiao Tong University (SJTU), China, and the M.S. degree from Purdue University, USA, both in mechanical engineering.
His research area is resilient operations of transportation systems under stochastic environments. He is interested in assessing negative impacts due to capacity/demand disruptions in transportation networks and designing resilient control policies, using ideas from stochastic processes, dynamic control, and optimization.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Amin}}]{Saurabh Amin} is Robert N. Noyce Career Development Associate Professor in the Department of Civil and Environmental Engineering, Massachusetts Institute of Technology (MIT). He received his Ph.D. in Systems Engineering from the University of California, Berkeley in 2011. His research focuses on the design and implementation of high confidence network control algorithms for infrastructure systems. 
%He works on robust diagnostics and control problems that involve using networked systems to facilitate the monitoring and control of large-scale critical infrastructures, including transportation, water, and energy distribution systems. 
%He also studies the effect of security attacks and random faults on the survivability of networked systems, and designs incentive-compatible control mechanisms to reduce network risks. 
He is a recipient of NSF CAREER award, and Google Faculty Research award. 
\end{IEEEbiography}
